Exploring Self-Supervised Multi-view Contrastive Learning for Speech Emotion Recognition with Limited Annotations

Recent advancements in Deep and Self-Supervised Learning (SSL) have led to substantial improvements in Speech Emotion Recognition (SER) performance, reaching unprecedented levels. However, obtaining sufficient amounts of accurately labeled data for training or fine-tuning the models remains a costly and challenging task. In this paper, we propose a multi-view SSL pre-training technique that can be applied to various representations of speech, including the ones generated by large speech models, to improve SER performance in scenarios where annotations are limited. Our experiments, based on wav2vec 2.0, spectral and paralinguistic features, demonstrate that the proposed framework boosts the SER performance, by up to 10% in Unweighted Average Recall, in settings with extremely sparse data annotations.

==> sections/2_related_work.tex <==
\section{Related Work}

==> tables/frozen.tex <==
\begin{table}[!t]
\centering
\scalebox{0.8}{
\begin{tabular}{clcc}
View                              & \multicolumn{1}{c}{F.E.} & UAR   & WA \\ \hline
\multirow{2}{*}{wav2vec 2.0}      &  \xmark                          & 63.11 & 61.36    \\
                                  &  \cmark                          & 55.43 & 53.97    \\ \hline
\multirow{2}{*}{Spectral} &  \xmark                          & 53.37 & 51.97    \\
                                  &  \cmark                         & 50.34 & 48.43    \\ \hline
\multirow{2}{*}{eGeMAPS-88}       &  \xmark                         & 52.96 & 49.16    \\
                                  &  \cmark                          & 49.65 & 48.97   
\end{tabular}}
\caption{Results for pre-trained models with frozen and tuned view-level encoders.}
\label{tab:frozen}
\end{table}

==> tables/temperature.tex <==
\begin{table*}[!t]
\scalebox{0.85}{
\begin{tabular}{cc|cc|cc|cc}
                             &             & \multicolumn{2}{c|}{wav2vec 2.0} & \multicolumn{2}{c|}{Spectral} & \multicolumn{2}{c}{eGeMAPS-88}  \\
Method                       & $\tau$ & UAR             & WA       & UAR               & WA         & UAR            & WA       \\ \hline
Supervised                   & -           & 62.11           & 59.43          & \textbf{53.39}    & \textbf{52.09}   & 49.97          & 48.1           \\ \hline
\multirow{4}{*}{Pairwise-CL} & 0.1         & 62.24           & \underline{61.51}    & 51.2              & 49.94            & \underline{51.38}    & \textbf{49.69} \\
                             & 0.25        & 62.38           & \textbf{61.59} & 50.69             & 50.17            & 50.77          & 47.99          \\
                             & 0.5         & \textbf{63.11}  & 61.36          & \underline{53.37}       & \underline{51.97}      & \textbf{52.96} & \underline{49.16}    \\
                             & 1.0         & 62.35           & 60.88          & 51.97             & 49.61            & 50.34          & 48.43         
\end{tabular}}
\caption{Performance metrics for models pre-trained with different values of temperature $\tau$ and fine-tuned on IEMOCAP-4. UAR refers to Unweighted Average Recall. For each view, we highlighted in bold and underlined the highest and the second-highest values.}
\label{tab:temp}
\end{table*}
